Expansivity and Roquette Groups

One looks at expansive subgroups in particular examples of Roquette groups. This study is motivated by the importance of expansive subgroups in the theory of stabilizing bisets highlighted in [BouThe]. In this paper we prove the non-existence of expansive subgroups with trivial G-core in different examples of Roquette groups G.

==> roquette.tex <==
\chapter{On Roquette Groups} \label{chapterroquette}
\renewcommand{\sectionmark}[1]{\markright{\uppercase{{#1}}}}
\sectionmark{CHAPTER $4$. On Roquette Groups}
\renewcommand{\sectionmark}[1]{\markright{\thesection\ \uppercase{{#1}}}}
As one has seen in the previous chapter we are going to put our attention on stabilizing bisets for Roquette groups. For this reason, one gives a brief description of Roquette groups. One finishes this chapter with a useful way to have Roquette groups as extension of known groups.
\begin{defn}{\text{}}
\begin{indice}
\item For a prime $p$, the \motdef{$p$-core of a finite group $G$}, denoted $O_p(G)$ \index{$O_p(G)$} , is defined to be its largest normal $p$-subgroup. 
\item \motdef{The Fitting subgroup of $G$}\index{Fitting subgroup}, denoted $F(G)$, is the product of the normal subgroups $O_p(G)$ for all primes $p$.
\item \motdef{The generalized Fitting subgroup of $G$}, denoted $F^{\star}(G)$, is the product of $F(G)$ and all quasisimple subnormal subgroups of $G$.
\end{indice} 
\end{defn}
\begin{defn}
Let $G$ be a group and $(G_i, 1 \leq i \leq m)$ a family of subgroups of $G$ for some integer $m$. Then $G$ is said to be a \motdef{central product}\index{central product} of the groups $G_i$, if
\begin{indice}
\item $G = {\ensuremath{\left\langle G_i \st 1 \leq i \leq m \right\rangle}}$,
\item $[G_i, G_j ] = 1$ for $i \neq j$. 
\end{indice}
In this case, we will write $G = G_1 \circ \dots \circ G_m$.
\end{defn}
\begin{rems}{\textbf{}}
\begin{maliste}
\item This definition implies in fact that all $G_i$ are normal subgroups of $G$. Indeed, let $x \in G_k$ and $y \in G$. By the first and the second conditions $y = y_1 \dots y_m$ with $y_i \in G_i$ for all $i$ and by the second one we have $[x,y] = [x, y_1 \dots y_m] = [x,y_k] \in G_k$. Therefore we have shown that $[G_k,G] \leq G_k$ which is equivalent to the statement.
\item Moreover, we have $G_i \cap G_j \subseteq Z(G)$ for $i \neq j$. Effectively, let $x$ be an element of $G_i \cap G_j$ and $y = y_1 \dots y_m$ an arbitrary element of $G$ like in the first point. Then $[x,y] = [x, y_1 \dots y_m] = [x,y_i]$ because $x \in G_i$, but $x$ is also in $G_j$ so $[x,y_i] = 1$, which shows that $G_i \cap G_j \subseteq Z(G)$. 
%Let $z$ be an element of $Z(G)$, especially, for all $i$, the element $z$ belongs to $Z(G_i)$, which is include in $G_i$ and shows the other inclusion. 
\item Let $G_1$ and $G_2$ be groups and let $Z(G_1)$, respectively $Z(G_2)$, be the center
of $G_1$, respectively $G_2$. Suppose that the two subgroups $Z(G_1)$ and $Z(G_2)$ are isomorphic. Given an isomorphism $\theta : Z(G_1) \rightarrow Z(G_2)$ we construct a central product $G_1 \circ G_2 := (G_1 \times G_2)/N$, where $N$ is the normal subgroup generated by the elements $\{(z, \theta(z^{-1})) \tq z \in Z(G_1)\}$. %Now it's an easy exercise to see that this definition is coherent with the above one.  
\end{maliste}
\end{rems}
%One needs to understand Roquette groups. 
Let $G$ be a Roquette group and denote by $F(G)$ the Fitting subgroup of $G$, which is the product of the normal subgroups $O_p(G)$ for all primes $p$. As $G$ is Roquette each $O_p(G)$ does not contain a characteristic abelian subgroup which is not cyclic. By theorem $4.9$ of \cite{Gor} on page $198$, such groups are known. More precisely, each subgroup $O_p(G)$ is the central product of an extraspecial group (possibly trivial) with a Roquette $p$-group. Such a group is called \motdef{quasi-Roquette}.
This description helps us to give a characterization of those groups.
\begin{prop} \label{charroquette}
A finite group $G$ is Roquette if and only if the Fitting subgroup is the direct product of quasi-Roquette groups and the action of $G$ on $F(G)$ doesn't fix an elementary abelian normal subgroup of rank at least $2$.
\end{prop}
\begin{proof}
If $G$ is Roquette, then it is straightforward that the Fitting subgroup is the direct product of quasi-Roquette groups and the action of $G$ on $F(G)$ doesn't fix an elementary abelian normal subgroup of rank at least $2$.

Suppose the Fitting subgroup is the direct product of quasi-Roquette groups and the action of $G$ on $F(G)$ doesn't fix an elementary abelian normal subgroup of rank at least $2$. Let $N$ be a normal elementary abelian $p$-subgroup of $G.$ One has to prove that $N$ is actually cyclic. Remark that $N$ is contained in $O_p(G)$ and so $N = N \cap O_p(G) \leq N \cap F(G) \leq F(G)$. Therefore $N$ is a normal subgroup of $F(G)$ fixed by the action of $G$, as $N$ is a normal subgroup of $G$. By assumption $N$ has to be cyclic.
\end{proof}

One also presents a way to have Roquette groups as extension of known groups. As one has described a Roquette group with is Fitting subgroup, one continues in this fashion.

Suppose $G$ is solvable. It is a well known fact that in this case $C_G(F(G)) \leq F(G)$. Therefore $G/F(G)$ injects into $\Out(F(G))$. Indeed consider the map $\phi : G \rightarrow \Out(F(G))$ sending an element $g$ to the class of the conjugation map $c_g$. Then $\ker\phi = \{  g \in G \st c_g \in \Inn(F(G)) \}$ which means that if $g \in \ker\phi$ there exists $h \in F(G)$ such that $c_g = c_h$. This is equivalent to saying that $\pg{h^{-1}g}x = x$ for all $x \in F(G)$, in other words $h^{-1}g$ belongs to $C_G(F(G))$ and therefore $g$ to $F(G) C_G(F(G)) = F(G)$. This shows that $\ker\phi \leq F(G)$ and the other inclusion is trivial. So one has the following exact sequence
\begin{figure}[h]
$$\xymatrix@1{1 \ar[r] & F(G) \ar[r] &G \ar[r] & S \ar[r] &1} $$
\end{figure}\\
where $S$ is a subgroup of $\Out(G)$.

In the case where $G$ is not solvable one has to replace $F(G)$ by the generalized Fitting group $F^{\star}(G)$ to have $C_G(F^{\star}(G)) \leq F^{\star}(G)$ and therefore $G/F^{\star}(G)$ injects into $\Out(F^{\star}(G))$.

\newpage
\chapter*{}

